Leveraging Application-Specific Knowledge for Energy-Efficient Deep Learning Accelerators on Resource-Constrained FPGAs

The growing adoption of Deep Learning (DL) applications in the Internet of Things has increased the demand for energy-efficient accelerators. Field Programmable Gate Arrays (FPGAs) offer a promising platform for such acceleration due to their flexibility and power efficiency. However, deploying DL models on resource-constrained FPGAs remains challenging because of limited resources, workload variability, and the need for energy-efficient operation. This paper presents a framework for generating energy-efficient DL accelerators on resource-constrained FPGAs. The framework systematically explores design configurations to enhance energy efficiency while meeting requirements for resource utilization and inference performance in diverse application scenarios. The contributions of this work include: (1) analyzing challenges in achieving energy efficiency on resource-constrained FPGAs; (2) proposing a methodology for designing DL accelerators with integrated Register Transfer Level (RTL) optimizations, workload-aware strategies, and application-specific knowledge; and (3) conducting a literature review to identify gaps and demonstrate the necessity of this work.

==> notes/note_1.tex <==
% \begin{itemize}
%     \item Prepare a paper of 10 pages (max.)
%     \item Participate in the review process
%     \item Present your work 
%     \item Identify contact points between your work and others
%     \item Build your social research network
%     \item Meet experts in your research domain
%     \item Enjoy the opportunity to improve your PhD work, overcome stipulations and learn from the experts
% \end{itemize}

% The papers should clearly motivate the PhD projects. Additionally, the key research questions driving the doctoral project should be outlined and the general approach or methodology used to address them should be described. Therefore, providing sufficient foundational information is essential to help readers understand the context. Finally, the papers should also discuss the current state of the doctoral research, such as progress made, any preliminary findings, or ongoing challenges.
